MAAS: Multi-modal Assignation for Active Speaker Detection

Active speaker detection requires a solid integration of multi-modal cues. While individual modalities can approximate a solution, accurate predictions can only be achieved by explicitly fusing the audio and visual features and modeling their temporal progression. Despite its inherent muti-modal nature, current methods still focus on modeling and fusing short-term audiovisual features for individual speakers, often at frame level. In this paper we present a novel approach to active speaker detection that directly addresses the multi-modal nature of the problem, and provides a straightforward strategy where independent visual features from potential speakers in the scene are assigned to a previously detected speech event. Our experiments show that, an small graph data structure built from a single frame, allows to approximate an instantaneous audio-visual assignment problem. Moreover, the temporal extension of this initial graph achieves a new state-of-the-art on the AVA-ActiveSpeaker dataset with a mAP of 88.8\%.

==> figures/LAN.tex <==
 \begin{figure}[t]
    \begin{center}
        \includegraphics[width=0.4\textwidth]{images/LAN.png}
    \end{center}
    \caption{\textbf{Local Assignation Graph} The basic graph for the multi-modal assignation is composed of one audio node and over video node for the facial features of each person visible on screen. The basic connectivity 
    }
    \label{fig:basicgraph}
\end{figure}


==> tables/supervisions.tex <==
\begin{table}[h!]
    \small
    \centering
    
    \begin{tabular}{c c c}
        \hline
        \textbf{Audio}  & \textbf{Visual}  &  \\
        \textbf{Supervision}  & \textbf{Supervision}  & \textbf{mAP} \\
        \hline 
        \xmark & \cmark & 88.5 \\
        \cmark & \cmark & \textbf{88.8} \\
        \hline
    \end{tabular}
     \caption{\textbf{Contribution of multi-modal Supervision.} 
    We control the contribution of the individual supervision sources, we see that the network only looses 0.3\% in performance if the audio supervision is lost. The direct audio supervision allows for slightly better estimation of speech events, thus refining the final active speaker assignation.
    }
    \label{tab:supervision}
\end{table}
